Efficient Nonmyopic Bayesian Optimization via One-Shot Multi-Step Trees

Bayesian optimization is a sequential decision making framework for optimizing expensive-to-evaluate black-box functions. Computing a full lookahead policy amounts to solving a highly intractable stochastic dynamic program. Myopic approaches, such as expected improvement, are often adopted in practice, but they ignore the long-term impact of the immediate decision. Existing nonmyopic approaches are mostly heuristic and/or computationally expensive. In this paper, we provide the first efficient implementation of general multi-step lookahead Bayesian optimization, formulated as a sequence of nested optimization problems within a multi-step scenario tree. Instead of solving these problems in a nested way, we equivalently optimize all decision variables in the full tree jointly, in a ``one-shot'' fashion. Combining this with an efficient method for implementing multi-step Gaussian process ``fantasization,'' we demonstrate that multi-step expected improvement is computationally tractable and exhibits performance superior to existing methods on a wide range of benchmarks.

==> content/experiments_old.tex <==
\section{Experiments}

We use $k$.PMS.$m$ to denote a pseudo $k$-step lookahead with $m$ Gauss-Hermite samples. 
We find $m=10$ is enough. 
\subsection{Simulated function}
We perform simulations on functions drawn from a Gaussian process. 
We follow the setting used in \cite{lam2016bayesian} and use a zero-mean \gp with square-exponential kernel with signal variance $\sigma_f^2=4$, input length scale $\ell=0.1$. Only difference is we use noise variance $\sigma_n^2=0.0001$ instead of 0.001 to simulate almost noiseless observations.  
We sample 100 functions defined on $\mathcal{X} = [0,1]^2$ from this \gp, and for each function, we start with one observation randomly sampled from $\mathcal{X}$, repeating for 100 times. 
We also set budget $T=15$.
Figure \ref{fig:simulation_results} shows the results. 

\begin{figure}
	\centering
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/sim_iter_aggregated.pdf}
		\subcaption{}
		\label{fig:gap_iter_curves}
	\end{subfigure}
	\hspace{.9cm}
    % \raisebox{-1ex}{%} 
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/sim_gap_time_scatter_scaled.pdf}
		\subcaption{}
		\label{fig:gap_time_error_bar}
	\end{subfigure}
	\caption{Results on simulated functions sampled from a \gp averaged over 100 functions and 100 repeats for each. 
	(a) Average \gap versus iteration. 
	(b) Average \gap versus time per iteration in log scale; error bars are also plotted.  
    $k$.PMS.$m$ means pseudo $k$-step lookahead with $m$ Gauss-Hermite samples. 
	}
	\label{fig:simulation_results}
\end{figure}

\subsection{Synthetic benchmark functions}
Following \cite{jiang2019efficient}, we test our algorithm on a set of nine ``challenging'' synthetic benchmark functions using exactly the same setting: start with $2d$ observations at uniformly random locations, then perform $20d$ iterations of \bo. 

\begin{table}[]
    \centering
    \caption{Average \gap over 100 repeats. Bold: best, blue: not significantly worse than best.}
    \label{tab:my_label}
\begin{tabular}{lllllllll}
\toprule
&{Rand} & {EI} & {12.EI.s} & {2.ts.10} & {2.ms.gh.10} & {3.ms.gh.10.5} & {2.wsms.gh.10} & {3.wsms.gh.10.5}\\\hline
{eggholder} & 0.498   &  0.613   &  \textbf{0.738  } &  0.600   &  0.602   &  0.672   &  0.478   &  0.536   \\  
{dropwave} & 0.486   &  0.439   &  \textit{\textcolor{blue}{0.598  }} &  \textit{\textcolor{blue}{0.584  }} &  0.495   &  0.499   &  \textit{\textcolor{blue}{0.545  }} &  \textbf{0.600  } \\  
{shubert} & 0.355   &  0.408   &  \textit{\textcolor{blue}{0.479  }} &  \textit{\textcolor{blue}{0.467  }} &  0.426   &  \textit{\textcolor{blue}{0.501  }} &  \textit{\textcolor{blue}{0.476  }} &  \textbf{0.507  } \\  
{rastrigin4} & 0.374   &  0.801   &  0.793   &  0.752   &  0.809   &  0.798   &  \textbf{0.851  } &  \textit{\textcolor{blue}{0.821  }} \\  
{ackley2} & 0.358   &  0.821   &  \textit{\textcolor{blue}{0.886  }} &  0.868   &  0.842   &  0.841   &  \textit{\textcolor{blue}{0.870  }} &  \textbf{0.895  } \\  
{ackley5} & 0.145   &  0.509   &  0.627   &  0.761   &  0.687   &  0.628   &  \textit{\textcolor{blue}{0.786  }} &  \textbf{0.793  } \\  
{bukin} & 0.600   &  0.849   &  0.829   &  \textbf{0.870  } &  0.850   &  0.851   &  \textit{\textcolor{blue}{0.862  }} &  \textit{\textcolor{blue}{0.862  }} \\  
{shekel5} & 0.038   &  0.286   &  0.358   &  0.394   &  0.432   &  0.389   &  \textit{\textcolor{blue}{0.827  }} &  \textbf{0.856  } \\  
{shekel7} & 0.045   &  0.268   &  0.412   &  0.454   &  0.437   &  0.425   &  \textit{\textcolor{blue}{0.825  }} &  \textbf{0.850  } \\  
{Average} & 0.322   &  0.555   &  0.635   &  0.639   &  0.620   &  0.623   &  \textit{\textcolor{blue}{0.725  }} &  \textbf{0.747  } \\  
\bottomrule
\end{tabular}
\end{table}

We show results in Figure \ref{fig:synthetic_results}.
12.\ei.s is the best performing options in \cite{jiang2019efficient}, which we include in the plot.
\begin{figure}
	\centering
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/synthetic_iter_aggregated.pdf}
		\subcaption{}
		\label{fig:gap_iter_curves}
	\end{subfigure}
	\hspace{.9cm}
    % \raisebox{-1ex}{%} 
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/synthetic_gap_time_scatter.pdf}
		\subcaption{}
		\label{fig:gap_time_error_bar}
	\end{subfigure}
	\caption{
	Results  on nice ``challenging'' synthetic benchmark functions averaged over 100 repeats.
	(a) Average \gap versus iteration. 
	(b) Average \gap versus time per iteration in log scale; error bars are also plotted.  
    $k$.PMS.$m$ means pseudo $k$-step lookahead with $m$ Gauss-Hermite samples. 
	}
	\label{fig:synthetic_results}
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/individual_synthetic_funcs/ackley5_iter_100_init_10.pdf}
		\subcaption{Ackley5}
		\label{fig:gap_iter_curves}
	\end{subfigure}
	\hspace{.9cm}
    % \raisebox{-1ex}{%} 
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/individual_synthetic_funcs/rastrigin4_iter_80_init_8.pdf}
		\subcaption{Rastrigin4}
		\label{fig:gap_time_error_bar}
	\end{subfigure}
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/individual_synthetic_funcs/dropwave_iter_40_init_4.pdf}
		\subcaption{Dropwave}
		\label{fig:gap_time_error_bar}
	\end{subfigure}
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/individual_synthetic_funcs/shubert_iter_40_init_4.pdf}
		\subcaption{Shubert}
		\label{fig:gap_time_error_bar}
	\end{subfigure}
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/individual_synthetic_funcs/shekel5_iter_80_init_8.pdf}
		\subcaption{Shekel5}
		\label{fig:gap_time_error_bar}
	\end{subfigure}
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/individual_synthetic_funcs/shekel7_iter_80_init_8.pdf}
		\subcaption{Shekel7}
		\label{fig:gap_time_error_bar}
	\end{subfigure}
	\caption{
	Individual functions.
	}
	\label{fig:synthetic_results}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/image.png}
    \caption{include 3-step EI, on nice synthetic functions.}
    \label{fig:my_label}
\end{figure}

\subsection{Hyperparameter tuning}
Following \cite{jiang2019efficient}, we test our algorithm on a set of seven hyperparameter tuning benchmark functions with exactly the same setting. 
Results are shown in Figure \ref{fig:real_results}.
Also included in the plot are the best variants of nonmyopic approximation 6.\ei.s, and two other nonmyopic baselines, \glasses and rollout, reported in \cite{jiang2019efficient}.
\begin{figure}
	\centering
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/real_iter_aggregated.pdf}
		\subcaption{}
		\label{fig:gap_iter_curves}
	\end{subfigure}
	\hspace{.9cm}
    % \raisebox{-1ex}{%} 
	\begin{subfigure}[b]{.45\textwidth}
		\includegraphics[width=\linewidth]{figures/real_gap_time_scatter.pdf}
		\subcaption{}
		\label{fig:gap_time_error_bar}
	\end{subfigure}
	\caption{
	Results  on seven real hyperparameter tuning functions average over 50 repeats.
	(a) Average \gap versus iteration. 
	(b) Average \gap versus time per iteration in log scale; error bars are also plotted.  
    $k$.PMS.$m$ means pseudo $k$-step lookahead with $m$ Gauss-Hermite samples. 
	}
	\label{fig:real_results}
\end{figure}

\subsection{Multi-step Knowledge Gradient}
Our derivation can apply to any utility function. 
In particular, where the function observation is noisy, it is often preferable to recommend the point with highest posterior mean, which indicates a utility function 
\begin{align}
    u_{\kg}(\data) = \max_{x\in \mathcal{X}} \mu_{f\given \data}(x). 
\end{align}
A one-step optimal policy with utility $u_{\kg}$ is known as the Knowledge Gradient (\kg) policy. 
We implement multi-step \kg using the one-shot approach, and show some results...

\subsection{Comparison with envolope-theorem-based implementation}


==> content/method.tex <==
\section{Efficient Nonmyopic Approximation}
\label{section:method}
We propose to adapt two ideas in related literature to achieve efficient and nonmyopic approximation of \eqref{eq:bellman_equation}.
\subsection{Achieving Nonmyopia via Non-Adaptive Approximation}
Inspired by recent advances in nonmyopic active search \cite{jiang2017efficient, jiang2018efficient}, we propose to use the optimal batch utility with the remaining budget as batch size to approximate the adaptive future utility: 
\begin{align}
        v_k(x \given \data) 
        &=
        v_1(x \given \data) 
        + 
        \E_y[ \max_{x'} v_{k-1}(x' \given \data_1 ) ]  \nonumber  \\
        & \Downarrow   \nonumber    \\
        v_k(x \given \data) 
        &\approx
        v_1(x \given \data) 
        + 
        \E_y[ \max_{X} V^{k-1}_1(X \given \data_1 ) ].  \label{eq:ensbo}
\end{align}
Comparing the above two equations closely, we replaced the adaptive value function $v_{k-1}$ by the non-adaptive value function $V^{k-1}_1$ with batch size $k-1$ and lookahead horizon 1, and pretend the second step is no longer a single point $x'$, but a set of points $X$ with $|X| = k-1$.
Note \eqref{eq:ensbo} can also be seen as a two-step lookahead utility where the second step is a batch with batch size being the remaining budget. 

Mathematically, \eqref{eq:ensbo} is a much tighter lower bound of the true objective \eqref{eq:bellman_equation} than existing one- or two-step lookahead, or existing heuristic methods such as \glasses \cite{gonzalez2016glasses} (more discussion in related work).

\subsection{Achieving Efficiency via One-Shot Optimization}
A naive implementation of \eqref{eq:ensbo} is to draw a set of $m$ samples $y^{(i)} \drawn \Pr(y\given x, \data), i=1,\dots, m$, and acquire a set of realizations of $\data_1$: $\data_1^{(i)} = \data \cup \{(x, y^{(i)}\}, i=1,\dots,m$.
For each $\data^{(i)}_1$, we update the \gp posterior $\Pr(Y\given X, \data^{(i)}_1) $ 
and optimize  
$X^{(i)} = \argmax_{X} V^{k-1}_1(X \given \data^{(i)}_1)$. 
Then $v_k(x\given \data)$ can be approximated via sample average:
\begin{equation}
    v_k(x \given \data) 
    \approx
    v_1(x\given \data) 
    + 
    \frac{1}{m} \sum_{i=1}^m V^{k-1}_1(X^{(i)} \given \data^{(i)}_1).  \label{eq:ensbo-sample-average}
\end{equation}
We can use any black-box optimization such as DIRECT or CMA-ES (covariance matrix adaptation evolution strategy) to optimize \eqref{eq:ensbo-sample-average}. 
It is also possible to adapt the envolope theorem-based technique introduced in \cite{wu2019practical} to optimize \eqref{eq:ensbo-sample-average} with gradient-based methods. However, this is still very expensive since every evaluation of \eqref{eq:ensbo-sample-average} involves solving $m$ high dimensional optimization problems. 

Inspired by recent advances in efficient implementation of the Knowledge Gradient acquisition function \cite{balandat2019botorch}, we propose a similar one-shot optimization technique for optimizing \eqref{eq:ensbo}.
The key idea is to move the max outside the expectation, and optimize $x$ and $X^{(i)}$'s jointly. 
That is, we solve the following optimization problem
\begin{align}
    \max_{x, X^{(1)}, \dots, X^{(m)} } 
    v_1(x\given \data) 
    + 
    \frac{1}{m} \sum_{i=1}^m V^{k-1}_1(X^{(i)} \given \data^{(i)}_1).  \label{eq:one-shot-ensbo}
\end{align}
Let $b=k-1$.
By moving the max outside the expectation, we turned a $d$ dimensional optimization of a very expensive objective (recall each evaluation involves $m$ optimizations of dimension $b\times d$) into a $d + m\times b \times d$ dimensional optimization where the objective is relatively easy to evaluate. 

We claim that mathematically this is an equivalent optimization. 
It can be understood by the simple relation 
$\max_{a,b} g(a, b) = \max_a \max_b g(a,b)$.
But the joint optimization is more efficient since we don't need to solve an expensive optimization problem to get the gradient w.r.t. $a$. 





==> content/related_old.tex <==
\section{Related Work}
\label{section:related}
The idea of one-shot optimization was recently proposed in \cite{balandat2019botorch} for optimizing the Knowledge Gradient (\kg) acquisition function \citep{wu2016parallel}, which also has a nested maximization (of the posterior mean). In this paper, we generalize this idea to full extent for efficient multi-step lookahead \bo.

While general multi-step lookahead \bo has never been attempted before due to its dauntingly high complexity, 
there are several earlier attempts on two-step lookahead \bo \citep{osborne2009gaussian, ginsbourger2010towards}.
The most related one is a recent development that made gradient-based optimization of two-step \ei possible \citep{wu2019practical}. 
% Recall the two-step lookahead value function (with Monte Carlo approximation) is as follows:
% \begin{align}
%     v_2(x\given \data) 
%     \approx 
%     v_1(x \given \data) 
%     +
%     \frac{1}{m_1}\sum_{i=1}^{m_1} \max_{x_2} v_1(x_2 \given \data, x, y^i).
% \end{align}
% Suppose $x_2^*$ achieves the maximum of $v_1(x_2\given \data, x, y_i)$. Plugging in $x_2^*$ we have 
% \begin{align}
%     v_2(x\given \data) 
%     \approx 
%     v_1(x \given \data) 
%     +
%     \frac{1}{m_1}\sum_{i=1}^{m_1} v_1(x_2^* \given \data, x, y^i).  \label{eq:envelope_two_step}
% \end{align}
% 
Their approach is precisely an implementation of the left hand side optimization in \eqref{eq:nested_vs_one_shot}, where maximizers of the second-stage value functions are first identified conditioned on each $y$ sample of the first stage, and then plugged back into the equation so that the $\max$ can be removed. 
If certain conditions are satisfied, this function is differentiable and admits unbiased gradient estimation based on the envelope theorem.
However, this method critically relies on the assumption that the located maximizers of the second-stage value functions are \emph{all global}. 
This assumption can be unrealistic, especially for high-dimensional problems, 
or requires too much computational effort (e.g., by requiring many restarts from different random initializations).
Note that any violation of this assumption would result in discontinuity of the objective, and the estimated gradients would be problematic.

Rollout is a classic approach to approximate dynamic programming \citep{sutton2018reinforcement}. 
\cite{lam2016bayesian,yue2019why} realized it for \bo. 
A two-step rollout is precisely the two-step lookahead, up to quadrature error.
When the rollout horizon is three or more, the rollout estimation of the expected utility is only a lower bound of the true multi-step expected utility, since it is simulating some \emph{base policy} instead of the \emph{optimal policy}.  
% Recently, \cite{yue2019why} provided some theoretical justifications of rollout and guidance on choosing the rolling horizon based on quantification of model misspecification error. 
% However, for similar reasons as discussed above for the two-step method, rollout is very expensive.
%to evaluate since it requires repeated optimization of the base acquisition function, and  such an expensive value function needs to be optimized (hence many evaluations).
%\cite{lee2020efficient} proposed a policy search heuristic to improve the efficiency by only optimizing the rollout function on the argmax of a set of base acquisition functions. 
% \cite{lee2020efficient} proposed efficient rollout strategies for \bo. Rollout is expensive because each evaluation of rollout value function requires repeated optimization of the base acquisition function, and then such an expensive value function needs to be optimized (hence many evaluations).
% One way to reduce of cost of each evaluation is to reduce the number of samples need to achieve a certain estimation accuracy. 
% Three commonly used variance reduction techniques are introduced in estimating the rollout value function: quasi Monte Carlo (qMC), common random number (CRN), and control variates.
% They further propose to not actually optimize the rollout value function, but instead perform policy search. Given a set of base policise, such as EI, PI, UCB etc., they roll out each policy on its argmax and then compare the rollout value, and simply apply the base policy with highest rollout value for this iteration.  

Another notable nonmyopic \bo policy is \glasses \citep{gonzalez2016glasses}, which also uses a similar non-adaptive approximation as \eno, i.e., uses a batch policy to simulate the future steps. 
However, they use a heuristic batch instead of the optimal batch, and their batch is not adaptive to the sample values of the first stage.
%The basic idea of the batch policy is to repeatedly optimize the \ei surface penalized by the proximity of previously added points, resulting in a diverse batch \citep{gonzalez2016batch}.
%It is similar to our proposed multi-step paths in the sense that it only has one path, but the path is heuristically constructed by artificially enforcing diversity. 
% The issues with \glasses is that it is still very expensive, and that one has to use black-box optimization method such as \acro{DIRECT} to maximize the acquisition function. 
All three methods discussed above share a similar procedure of repeated nested optimization for each evaluation of the acquisition function, hence very expensive to optimize. 


Recently \cite{jiang2019binoculars} proposed an 
efficient nonmyopic approach called \binoc. 
The idea is surprisingly simple: first compute an optimal batch, then select one point from the batch. This heuristic is justified by the fact that any point in the batch maximizes a lower bound of the true expected utility, tighter than \glasses. 
%Extensive experiments show its superior performance over existing myopic and nonmyopic methods, 
Empirical results show that \binoc compares favorably with existing myopic and nonmyopic methods in terms of efficiency and performance,  including rollout and \glasses. 
In this paper, we will mainly compare with \binoc. 

Our proposed \eno can be considered as an improved version of \binoc in the sense that it is maximizing an even tighter lower bound by moving the maximization inside the expectation (see Table \ref{table:comparison_of_bounds}). 
%\binoc corresponds to moving the remaining expectation over $\epsilon$ in~\eqref{eq:lower_bound} inside the maximization terms. 
The idea behind \eno has been successfully applied in \emph{active search} \citep{jiang2017efficient, jiang2018efficient}, a sequential experimental design setting with discrete domain and binary outcome, and a cumulative utility. 
While relatively easy to compute in the discrete case, it is quite expensive in the continuous setting if computed in a naive manner. Our one-shot optimization approach provides an efficient alternative.

We summarize all the nonmyopic methods discussed in this paper in Table~\ref{table:comparison_of_bounds}, in which we also present comparisons of the tightness of the lower bounds.

\begin{table}[t]
    \centering
    \caption{Summary of and comparison among the nonmyopic approaches discussed in this paper. 
    Notations: for \glasses, $X_g$ is a heuristically constructed batch; note it does not depend on $y$; for rollout, $r_1(x\given \data) = v_1(x \given \data)$, 
    and $\pi(\data_1) = \argmax_x v_1(x \given \data_1)$ is the base policy. Recall $\data_1 = \data \cup \{(x, y)\}$.
    }
    \label{table:comparison_of_bounds}
    \def\arraystretch{1.3}
    \vspace{1ex}
\begin{tabular}{lll}
\toprule
method  &   acquisition function  & reference   \\ 
\hline
multi-step  & $v_1(x\given \data) + \E_y [  \textstyle{  \max_{x'} } v_{k-1}(x' \given \data_1) ]$   & Ours \\
    \eno & $v_1(x\given \data) + \E_y [ \textstyle{  \max_X } V^{k-1}_1(X \given \data_1) ]$  & Ours\\
    \binoc & $v_1(x\given \data) + \textstyle{ \max_X } \E_y [ V^{k-1}_1(X \given \data_1) ]$  & \cite{jiang2019binoculars} \\
    \glasses & $v_1(x\given \data) + \E_y [ V^{k-1}_1(X_g \given \data_1) ]$   & \cite{gonzalez2016glasses} \\
    rollout & $r_k(x\given \data) = r_1(x\given\data) + \E_y[ r_{k-1}(\pi(\data_1) \given \data_1) ]$  & \cite{lam2016bayesian} \\ 
    two-step & $v_1(x\given \data) + \E_y [  \textstyle{  \max_{x'} } v_{1}(x' \given \data_1) ]$  & \cite{wu2019practical} \\
    one-step   & $v_1(x\given \data) + 0 $  & \cite{movckus1975bayesian} \\ 
        \hline 
        \multirow{3}{*}{relationships (when $k\ge2$)}  
                & \multicolumn{2}{l}{multi-step $\ge$ \eno $\ge$ \binoc $\ge$ \glasses $\ge$ one-step;}   \\
                & multi-step $\ge$ rollout $\ge$ two-step $\ge$ one-step;  & \\
                & \eno $\ge$ two-step. & \\
            \bottomrule
    \end{tabular}
\end{table}
% \begin{align}
% \text{Optimal: } & v_1(x\given \data) + \E_y [  \textstyle{  \max_{x'} } v_{k-1}(x' \given \data, x, y) ].  \label{eq:true_expected_utility}  \\
%     \text{\eno: } & v_1(x\given \data) + \E_y [ \textstyle{  \max_X } V^{k-1}_1(X \given \data, x, y) ], \\
%     \text{\binoc: } & v_1(x\given \data) + \textstyle{ \max_X } \E_y [ V^{k-1}_1(X \given \data, x, y) ], \\
%     \text{\glasses: } & v_1(x\given \data) + \E_y [ V^{k-1}_1(X_g \given \data, x, y) ] \text{ ($X_g$ is a heuristic batch).} 
% \end{align}
Finally, we would like to point out the connections between batch construction and nonmyopic approximations in general sequential experimental design.
As indicated earlier, if we use Gauss-Hermite quadrature with a single sample, we in fact just use the mean of the Gaussian distribution. 
This fact relates the ``multi-step path'' to some of the notable batch construction heuristics such as Kriging Believer \citep{ginsbourger2010kriging}, or \acro{GP-BUCB} \citep{desautels2014parallelizing}, where we fantasize (or ``hallucinate'' as is called in \cite{desautels2014parallelizing}) the posterior mean and continue simulating next steps as if it were the actual observed value. 
Such connections between batch construction and nonmyopic approximations are not coincidental; as we have seen in Table \ref{table:comparison_of_bounds}, most of the nonmyopic approaches use a batch policy as a subroutine, and batch policies are often based on multi-step simulations of a sequential policy \citep{azimi2010batch, azimi2012batch, jiang2018efficient}. 


==> tables/synthetic_functions_gap_ttest.tex <==
% \begin{tabular}{lllllllll}
% \toprule
% &{EI} & {ETS} & {12.EI.s} & {2-step'} & {3-step'} & {2-step} & {3-step} & {4-step}\\\hline
% {eggholder} & 0.627   &  0.645   &  \textbf{0.736  } &  0.602   &  0.672   &  0.478   &  0.536   &  0.577   \\  
% {dropwave} & 0.429   &  \textit{\textcolor{blue}{0.585  }} &  \textit{\textcolor{blue}{0.606  }} &  0.495   &  0.499   &  0.545   &  \textit{\textcolor{blue}{0.600  }} &  \textbf{0.635  } \\  
% {shubert} & 0.376   &  0.482   &  \textit{\textcolor{blue}{0.515  }} &  0.426   &  \textit{\textcolor{blue}{0.501  }} &  0.476   &  \textit{\textcolor{blue}{0.507  }} &  \textbf{0.562  } \\  
% {rastrigin4} & 0.816   &  0.482   &  0.790   &  0.809   &  0.798   &  \textbf{0.851  } &  \textit{\textcolor{blue}{0.821  }} &  \textit{\textcolor{blue}{0.826  }} \\  
% {ackley2} & 0.808   &  0.855   &  \textbf{0.902  } &  0.842   &  0.841   &  \textit{\textcolor{blue}{0.870  }} &  \textit{\textcolor{blue}{0.895  }} &  \textit{\textcolor{blue}{0.888  }} \\  
% {ackley5} & 0.576   &  0.528   &  0.703   &  0.687   &  0.628   &  \textit{\textcolor{blue}{0.786  }} &  \textit{\textcolor{blue}{0.793  }} &  \textbf{0.804  } \\  
% {bukin} & 0.841   &  0.843   &  0.842   &  \textit{\textcolor{blue}{0.850  }} &  \textit{\textcolor{blue}{0.851  }} &  \textbf{0.862  } &  \textit{\textcolor{blue}{0.862  }} &  \textit{\textcolor{blue}{0.861  }} \\  
% {shekel5} & 0.349   &  0.129   &  0.496   &  0.432   &  0.389   &  \textit{\textcolor{blue}{0.827  }} &  \textbf{0.856  } &  \textit{\textcolor{blue}{0.847  }} \\  
% {shekel7} & 0.363   &  0.157   &  0.506   &  0.437   &  0.425   &  \textit{\textcolor{blue}{0.825  }} &  \textbf{0.850  } &  0.775   \\  
% \hline 
% {Ave. \gap} & 0.576   &  0.530   &  0.677   &  0.620   &  0.623   &  0.725   &  \textit{\textcolor{blue}{0.747  }} &  \textbf{0.753  } \\  
% Ave. time/iter & 1.157 & 1949. & 25.74 & 7.772 & 40.78 & 7.163 & 39.53 & 197.7 \\
% \bottomrule
% \end{tabular}

\begin{tabular}{llllllllll}
\toprule
&{EI} & {ETS} & {12.EI.s} & {2-step'} & {2-step} & {3-step} & {4-step} & {4-path} & {12-\eno}\\\hline
{eggholder} & 0.627   &  0.647   &  \textbf{0.736  } &  0.602   &  0.478   &  0.536   &  0.577   &  0.567   &  0.661   \\  
{dropwave} & 0.429   &  0.585   &  0.606   &  0.495   &  0.545   &  0.600   &  0.635   &  \textbf{0.731  } &  0.673   \\  
{shubert} & 0.376   &  \textit{\textcolor{blue}{0.487  }} &  \textit{\textcolor{blue}{0.515  }} &  0.426   &  0.476   &  \textit{\textcolor{blue}{0.507  }} &  \textbf{0.562  } &  \textit{\textcolor{blue}{0.560  }} &  \textit{\textcolor{blue}{0.494  }} \\  
{rastrigin4} & 0.816   &  0.491   &  0.790   &  0.809   &  \textbf{0.851  } &  0.821   &  0.826   &  \textit{\textcolor{blue}{0.837  }} &  \textit{\textcolor{blue}{0.837  }} \\  
{ackley2} & 0.808   &  0.856   &  \textit{\textcolor{blue}{0.902  }} &  0.842   &  0.870   &  0.895   &  0.888   &  \textbf{0.931  } &  0.847   \\  
{ackley5} & 0.576   &  0.516   &  0.703   &  0.687   &  0.786   &  0.793   &  0.804   &  \textbf{0.875  } &  \textit{\textcolor{blue}{0.856  }} \\  
{bukin} & \textit{\textcolor{blue}{0.841  }} &  \textit{\textcolor{blue}{0.843  }} &  0.842   &  \textit{\textcolor{blue}{0.850  }} &  \textbf{0.862  } &  \textit{\textcolor{blue}{0.862  }} &  \textit{\textcolor{blue}{0.861  }} &  \textit{\textcolor{blue}{0.852  }} &  0.836   \\  
{shekel5} & 0.349   &  0.132   &  0.496   &  0.432   &  \textit{\textcolor{blue}{0.827  }} &  \textbf{0.856  } &  \textit{\textcolor{blue}{0.847  }} &  0.718   &  0.799   \\  
{shekel7} & 0.363   &  0.159   &  0.506   &  0.437   &  \textit{\textcolor{blue}{0.825  }} &  \textit{\textcolor{blue}{0.850  }} &  0.775   &  0.776   &  \textbf{0.866  } \\   
\bottomrule
{Average} & 0.576   &  0.524   &  0.677   &  0.620   &  0.725   &  \textit{\textcolor{blue}{0.747  }} &  \textit{\textcolor{blue}{0.753  }} &  \textit{\textcolor{blue}{0.761  }} &  \textbf{0.763  } \\  
Ave. time & 1.157 & 1949. & 25.74 & 7.772 & 7.163 & 39.53 & 197.7 & 17.50 & 15.61 \\
\bottomrule
\end{tabular}
